Parametric Shadow Control for Portrait Generation in Text-to-Image Diffusion Models

Text-to-image diffusion models excel at generating diverse portraits, but lack intuitive shadow control. Existing editing approaches, as post-processing, struggle to offer effective manipulation across diverse styles. Additionally, these methods either rely on expensive real-world light-stage data collection or require extensive computational resources for training. To address these limitations, we introduce Shadow Director, a method that extracts and manipulates hidden shadow attributes within well-trained diffusion models. Our approach uses a small estimation network that requires only a few thousand synthetic images and hours of training-no costly real-world light-stage data needed. Shadow Director enables parametric and intuitive control over shadow shape, placement, and intensity during portrait generation while preserving artistic integrity and identity across diverse styles. Despite training only on synthetic data built on real-world identities, it generalizes effectively to generated portraits with diverse styles, making it a more accessible and resource-friendly solution.

==> figure/Fig_01_Teaser.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figure/fig_01_Teaser.pdf}
    \caption{Shadow Director allows users to intuitively customize shadow effects on stylized portraits without trial-and-error prompt engineering. It provides control over shadow intensity, from weaker to stronger shadows, and enables shadow placement and shaping through user-defined masks or lighting positions}
    \label{fig:dataset}
\end{figure*}





==> figure/Fig_04_Ablation_Necessity_of_SD.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/fig_04_Ablation_Necessity_of_SD.pdf}
    \caption{\textbf{Necessity of Design in Shadow Director.} }
    \label{fig:ablation_visual}
\end{figure}

